A Strong and Reproducible Object Detector with Only Public Datasets

This work presents Focal-Stable-DINO, a strong and reproducible object detection model which achieves 64.6 AP on COCO val2017 and 64.8 AP on COCO test-dev using only 700M parameters without any test time augmentation. It explores the combination of the powerful FocalNet-Huge backbone with the effective Stable-DINO detector. Different from existing SOTA models that utilize an extensive number of parameters and complex training techniques on large-scale private data or merged data, our model is exclusively trained on the publicly available dataset Objects365, which ensures the reproducibility of our approach.

==> images_tex/coco_sota_minival.tex <==
\begin{figure}[h]
    \centering
    % \vspace{-0.2cm}
    \includegraphics[width=0.98\linewidth]{resources/coco_sota_minival.pdf}
    % \vspace{-0.1cm}
    \caption{Comparison with SoTA on COCO \texttt{val2017}. Circle size indicates the model size. "\#" means using TTA (Test Time Augmentation)}
    \label{fig:coco_sota_minival}
    % \vspace{-0.4cm}
\end{figure}

==> images_tex/vis.tex <==
\begin{figure*}[htbp]
\centering
\resizebox{0.84\textwidth}{!}{%
\subfigure{
\begin{minipage}[t]{0.5\linewidth}
    \subfigure{
    \begin{minipage}[t]{1.0\linewidth}
    \centering
    \includegraphics[width=\linewidth]{resources/pos_case/000000003934.jpg}
    % \caption{predicted boxes.}
    \end{minipage}
    }
    \subfigure{
    \begin{minipage}[t]{1.0\linewidth}
    \centering
    \includegraphics[width=\linewidth]{resources/pos_case/000000005037.jpg}
    % \caption{initial anchor boxes.}
    \end{minipage}
    }
    \subfigure{
    \begin{minipage}[t]{1.0\linewidth}
    \centering
    \includegraphics[width=\linewidth]{resources/pos_case/000000005992.jpg}
    % \caption{anchor boxes after the first decoder.}
    \end{minipage}
    }
    % \caption{Results of MDETR.}
    \subfigure{
    \begin{minipage}[t]{1.0\linewidth}
    \centering
    \includegraphics[width=\linewidth]{resources/pos_case/000000007386.jpg}
    % \caption{anchor boxes after the first decoder.}
    \end{minipage}
    }
    % \subfigure{
    % \begin{minipage}[t]{1.0\linewidth}
    % \centering
    % \includegraphics[width=\linewidth]{resources/pos_case/000000023034.jpg}
    % % \caption{anchor boxes after the first decoder.}
    % \end{minipage}
    % }
\end{minipage}
}%
% \subfigure{
% \begin{minipage}[t]{0.5\linewidth}
%     \subfigure{
%     \begin{minipage}[t]{1.0\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{resources/pos_case/000000006471.jpg}
%     % \caption{predicted boxes.}
%     \end{minipage}
%     }
%     \subfigure{
%     \begin{minipage}[t]{1.0\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{resources/pos_case/000000007108.jpg}
%     % \caption{initial anchor boxes.}
%     \end{minipage}
%     }
%     % \subfigure{
%     % \begin{minipage}[t]{1.0\linewidth}
%     % \centering
%     % \includegraphics[width=\linewidth]{resources/pos_case/000000007281.jpg}
%     % % \caption{anchor boxes after the first decoder.}
%     % \end{minipage}
%     % }
%     \subfigure{
%     \begin{minipage}[t]{1.0\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{resources/pos_case/000000007888.jpg}
%     % \caption{anchor boxes after the first decoder.}
%     \end{minipage}
%     }
%     \subfigure{
%     \begin{minipage}[t]{1.0\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{resources/pos_case/000000023230.jpg}
%     % \caption{anchor boxes after the first decoder.}
%     \end{minipage}
%     }
%     \subfigure{
%     \begin{minipage}[t]{1.0\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{resources/pos_case/000000037988.jpg}
%     % \caption{anchor boxes after the first decoder.}
%     \end{minipage}
%     }
%     % \caption{Results of MDETR.}
% \end{minipage}
% }%
}
\centering
\caption{Visualizations of model outputs.\textbf{SHILONG TODO: refine the figure}}
\label{fig:vis}
\end{figure*}

==> table_tex/data.tex <==
\begin{table*}[ht]
\centering\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.5}
\footnotesize
\vspace{-0mm}
\resizebox{1.0\columnwidth}{!}{%
\begin{tabular}{ccc}
\shline
Data & Description & Data Size \\
\shline
IN-1K & ImageNet-1K  & 1M image data \\
\shline
\end{tabular}
\vspace{-0.2cm}
\caption{{The details of training data.}}
\label{tab:data_detail}}
\end{table*}

